ConViT: Improving Vision Transformers with Soft Convolutional Inductive Biases

Convolutional architectures have proven extremely successful for vision tasks. Their hard inductive biases enable sample-efficient learning, but come at the cost of a potentially lower performance ceiling. Vision Transformers (ViTs) rely on more flexible self-attention layers, and have recently outperformed CNNs for image classification. However, they require costly pre-training on large external datasets or distillation from pre-trained convolutional networks. In this paper, we ask the following question: is it possible to combine the strengths of these two architectures while avoiding their respective limitations? To this end, we introduce gated positional self-attention (GPSA), a form of positional self-attention which can be equipped with a ``soft" convolutional inductive bias. We initialise the GPSA layers to mimic the locality of convolutional layers, then give each attention head the freedom to escape locality by adjusting a gating parameter regulating the attention paid to position versus content information. The resulting convolutional-like ViT architecture, ConViT, outperforms the DeiT on ImageNet, while offering a much improved sample efficiency. We further investigate the role of locality in learning by first quantifying how it is encouraged in vanilla self-attention layers, then analysing how it is escaped in GPSA layers. We conclude by presenting various ablations to better understand the success of the ConViT. Our code and models are released publicly at https://github.com/facebookresearch/convit.

==> main_text_old.tex <==

\section{Introduction}

The success of deep learning over the last decade has largely been fueled by models with strong inductive biases, allowing efficient training across domains~\cite{mitchell1980need,goodfellow_deep_2016}. The use of Convolutional Neural Networks (CNNs)~\cite{lecun1998gradient,lecun1989backpropagation}, which have become ubiquitous in computer vision since the success of AlexNet in 2012~\cite{krizhevsky2017imagenet}, epitomizes this trend. Inductive biases are hard-coded into the architectural structure of CNNs in the form of two strong constraints on the weights: locality and weight sharing. By encouraging translation equivariance (without pooling layers) and translation invariance (with pooling layers)~\cite{scherer_evaluation_2010,schmidhuber_deep_2015,goodfellow_deep_2016}, the convolutional inductive bias makes models more sample-efficient and parameter-efficient~\cite{simoncelli2001natural,ruderman1994statistics}. Similarly, for sequence-based tasks, recurrent networks with hard-coded memory cells have been shown to simplify the learning of long-range dependencies (LSTMs) and outperform vanilla recurrent neural networks in a variety of settings~\cite{gers1999learning,sundermeyer_lstm_2012,greff_lstm_2017}.

However, the rise of models based purely on attention in recent years calls into question the necessity of hard-coded inductive biases. First introduced as an add-on to recurrent neural networks for Sequence-to-Sequence models~\cite{bahdanau2014neural}, attention has led to a breakthrough in Natural Language Processing through the emergence of Transformer models, which rely solely on a particular kind of attention: Self-Attention (SA) \cite{vaswani2017attention}. The strong performance of these models when pre-trained on large datasets has quickly led to Transformer-based approaches becoming the default choice over recurrent models like LSTMs~\cite{devlin2018bert}.

In vision tasks, the locality of CNNs impairs the ability to capture long-range dependencies, whereas attention does not suffer from this limitation. \citet{chen20182} and ~\citet{bello2019attention} leveraged this complementarity by augmenting convolutional layers with attention. More recently, ~\citet{ramachandran2019stand} ran a series of experiments replacing some or all convolutional layers in ResNets with attention, and found the best performing models used convolutions in early layers and attention in later layers. The Vision Transformer (ViT), introduced by ~\citet{dosovitskiy2020image}, entirely dispenses with the convolutional inductive bias by performing SA across embeddings of patches of pixels. The ViT is able to match or exceed the performance of CNNs but requires pre-training on vast amounts of data. More recently, the Data-efficient Vision Transformer (DeiT)~\cite{touvron2020training} was able to reach similar performances without any pre-training on supplementary data, instead relying on Knowledge Distillation~\cite{hinton2015distilling} from a convolutional teacher.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/phase_space.pdf}
    \caption{\textbf{Soft inductive biases can help models learn without being restrictive.} Hard inductive biases, such as the architectural constraints of CNNs, can greatly improve the sample-efficiency of learning, but can become constraining when the size of the dataset is not an issue. The soft inductive biases introduced by the ConViT avoid this limitation by vanishing away when not required. 
    }
    \label{fig:phase_space}
\end{figure}


\paragraph{Soft inductive biases}

The recent success of the ViT demonstrates that while convolutional constraints can enable strongly sample-efficient training in the small-data regime, they can also become limiting as the dataset size is not an issue. In data-plentiful regimes, hard inductive biases can be overly restrictive and \textit{learning} the most appropriate inductive bias can prove more effective. The practitioner is therefore confronted with a dilemma between using a convolutional model, which has a high performance floor but a potentially lower performance ceiling due to the hard inductive biases, or a self-attention based model, which has a lower floor but a higher ceiling. This dilemma leads to the following question: can one get the best of both worlds, and obtain the benefits of the convolutional inductive biases without suffering from its limitations?

In this direction, one successful approach is the combination of the two architectures in ``hybrid" models. These models, which interleave or combine convolutional and self-attention layers, have fueled successful results in a variety of tasks ~\cite{carion2020end,hu2018relation,ramachandran2019stand,chen2020uniter,locatello2020object,sun2019videobert,srinivas20201bottleneck,wu_visual_2020}. While this method is an interesting compromise, it enforces the hard convolutional inductive bias and its associated limitations inside the Transformer. Another approach is that of Knowledge Distillation~\cite{hinton2015distilling}, which has recently been applied to transfer the inductive bias of a convolutional teacher to a student transformer~\cite{touvron2020training}.

\paragraph{Contribution}
In this work, we present a new method to ``softly" introduce a convolutional inductive bias directly into SA layers, as an attempt to bridge the gap between CNNs and Transformers. 
%Our approach builds on the idea, first introduced in~\citet{cordonnier2019relationship}, that SA layers with positional embeddings are capable of expressing convolutional layers, and tend to do so in practice. 
We make the following contributions:
\begin{enumerate}[noitemsep,labelindent=0pt]
    \item We show quantitatively that SA layers are pulled towards locality in the early stages of training, then escape locality later on in training. 
    \item Motivated by this observation, we present a new form of SA layer, named \emph{gated positional self-attention} (GPSA), which we initialize as a convolutional layer, then encourage to recover expressivity by adjusting a \emph{gating parameter}.
    \item We then perform experiments based on the DeiT~\cite{touvron2020training}, with a certain number of SA layers replaced by GPSA layers. The resulting Convolutional Vision Transformer (ConViT) outperforms the DeiT (Fig.~\ref{fig:sota}) with less parameters, and offers better sample-efficiency (Tab.~\ref{tab:perfs}). 
\end{enumerate}

Overall, our work demonstrates the effectiveness of soft inductive biases, especially in the highly underspecified regime in which modern networks typically operate (see Fig.~\ref{fig:phase_space}), and motivates the exploration of further methods to induce soft inductive biases. 

\begin{table}[t]
    \footnotesize
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
    Train set & DeiT & ConViT & Rel. improv. (\%) \\
    \hline
    10\% & 45.9 & \textbf{58.6} & 27.5\\
    30\% & 63.1 & \textbf{73.2} & 15.9\\
    100\% &79.1 & \textbf{82.2} & 3.9 \\
    % 10\% & 45.9 / 69.3 & \textbf{58.6 / 79.9} & 27.5 / 15.3\\
    % 30\% & 63.1 / 83.6 & \textbf{73.2 / 89.6} & 15.9 / 7.4\\
    % 100\% &79.1 / 94.4 & \textbf{82.2 / 95.9} & 3.9 /  1.6\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{The convolutional inductive bias strongly improves sample efficiency.} We compare the top-1  accuracy of our ConViT-S with that of the DeiT~\cite{touvron2020training} of same architecture (see Tab.~\ref{tab:sizes} for details). Both models are trained on a subsampled version of ImageNet-1k, where we only keep a fraction $f\in\{0.1,0.3,1\}$ of the images of each class for training.}
    \label{tab:perfs}
\end{table}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{.49\columnwidth}
    \includegraphics[width=\linewidth]{figs/model_size_CIFAR100_intro.pdf}    
    \caption{CIFAR100}
    \end{subfigure}
    \begin{subfigure}[b]{.49\columnwidth}
    \includegraphics[width=\linewidth]{figs/model_size_IMNET_intro.pdf}    
    \caption{ImageNet-1k}
    \end{subfigure}
    % \includegraphics[width=.5\columnwidth]{figs/data_size_intro.pdf}
    \caption{\textbf{The ConViT performs well both on small and large datasets}. We compare the top-1 accuracies of our three ConViT models (Tab.~\ref{tab:sizes}) with those of other ViTs (diamonds) and CNNs (squares) on both CIFAR100 and ImageNet. Data used for CIFAR100:~\cite{zagoruyko2016wide,huang2017densely,zhao2020splitnet}. Data used for ImageNet:~\cite{he2016deep,tan2019efficientnet,touvron2020training,wu_visual_2020,yuan2021tokens}.}
    \label{fig:sota}
\end{figure}

\giulio{This last sentence coudl be expanded a bit and here we can refer to Fig.1} \levent{indeed, DeiT is a bit of a specific choice and would not be directly familiar for many people, we could add a few sentences justifying the choice of DeiT and describing it's core contribution in a sentence (which we already expand a bit in the `related work' session @hugo)}

\paragraph{Related work}
\matthew{I feel like there's also an angle of our work being relevant to the broader goal of making models more sample-efficient. Perhaps could start general and move towards the two more specific examples you describe below.}

Our work is motivated by combining the recent success of pure Transformer models ~\cite{dosovitskiy2020image} with the formalized relationship between SA and convolution. Indeed, \citet{cordonnier2019relationship} showed that a SA layer with $N_h$ heads can express a convolution of kernel size $\sqrt N_h$, if each head focuses on one of the pixels in the kernel patch. By investigating the qualitative aspect of attention maps of models trained on CIFAR-10, it is shown that SA layers with relative positional encodings naturally converge towards convolutional-like configurations, suggesting that some degree of convolutional inductive bias is desirable.

Conversely, the restrictiveness of hard locality constraints has been proven by~\citet{elsayed2020revisiting}. A breadth of approaches have been taken to imbue CNN architectures with non-locality ~\cite{hu_gather-excite_2018,hu_squeeze-and-excitation_2018,wang_non-local_2018,wu_visual_2020}. Another line of research is to induce a convolutional inductive bias is different architectures. For example, \citet{neyshabur2020towards} uses a regularization method to encourage fully-connected networks (FCNs) to learn convolutions from scratch throughout training. 

Most related to our approach, \citet{d2019finding} explored a method to initialize FCNs networks as CNNs. This enables the resulting FCN to reach much higher performance than achievable with standard initialization. Moreover, if the FCN is initialized from a partially trained CNN, the recovered degrees of freedom allow the FCN to outperform the CNN it stems from. This method relates more generally to ``warm start" approaches such as those used in spiked tensor models \cite{anandkumar2016homotopy}, where a smart initialization, containing prior information on the problem, is used to ease the learning task.

% \paragraph{Reproducibility}
% We provide an open-source implementation of our method. It is available at \url{https://github.com/facebookresearch/convit}.

%Our method of initializing self-attention layers as convolutions is, to the best of our knowledge, novel. 

\section{Background}

We begin by introducing the basics of SA layers, and show how positional attention can allow SA layers to express convolutional layers.

\paragraph{Multi-head self-attention} \label{sec:mhsa}

The attention mechanism is based on a trainable associative memory with (key, query) vector pairs. A sequence of $L_1$ ``query" embeddings $\boldsymbol Q\in \mathbb{R}^{L_1\times D_{h}}$ is matched against another sequence of $L_2$ ``key" embeddings $\boldsymbol K\in\mathbb{R}^{L_2\times D_{h}}$ using inner products. The result is an attention matrix whose entry $(ij)$ quantifies how semantically ``relevant" $\boldsymbol Q_i$ is to $\boldsymbol K_j$:
\begin{equation}
    \boldsymbol A = \operatorname{softmax}\left(\frac{\boldsymbol Q \boldsymbol K^\top}{\sqrt {D_{h}}}\right) \in \mathbb{R
}^{L_1\times L_2}.
    \label{eq:attention}
\end{equation}

Self-attention is a special case of attention where a sequence is matched to itself, to extract the semantic dependencies between its parts. In the ViT, the queries and keys are linear projections of the embeddings of $16\times 16$ pixel patches $\boldsymbol X\in\mathbb{R}^{L\times D_{emb}}$. Hence, we have $\boldsymbol Q = \boldsymbol W_{qry} \boldsymbol X$ and $\boldsymbol K = \boldsymbol W_{key} \boldsymbol X$, where $\boldsymbol{W}_{key}, \boldsymbol{W}_{qry}\in\mathbb R^{D_{emb}\times D_{h}}$. 

Multi-head SA layers use several self-attention heads in parallel to allow the learning of different kinds of interdependencies. They take as input a sequence of $L$ embeddings of dimension $D_{emb} = N_h D_h$, and output a sequence of $L$ embeddings of the same dimension through the following mechanism:
\begin{align}
    \operatorname{MSA}(\boldsymbol{X}):=\underset{h \in\left[N_{h}\right]}{\operatorname{concat}}\left[\text{SA}_{h}(\boldsymbol{X})\right] \boldsymbol{W}_{out}+\boldsymbol{b}_{out},
\end{align}
where $\boldsymbol{W}_{out}\in\mathbb R^{D_{emb} \times D_{emb}}, b_{out}\in\mathbb R^{D_{emb}}$. Each self-attention head $h$ performs the following operation:  
\begin{align}
    \text{SA}_h(\boldsymbol{X}) := \boldsymbol{A}^h \boldsymbol{X} \boldsymbol{W}_{val}^h,
\end{align}
where $\boldsymbol W_{val}^h \in R^{D_{emb} \times D_h}$ is the \emph{value} matrix.

However, in the vanilla form of Eq.~\ref{eq:attention}, SA layers are position-agnostic: they do not know how the patches are located according to each other. To incorporate positional information, there are several options. One is to add some positional information to the input at embedding time, before propagating it through the SA layers: ~\cite{dosovitskiy2020image} use this approach in their ViT. Another possibility is to replace the vanilla SA with positional self-attention (PSA), using embeddings $\boldsymbol r_{ij}$ of the relative position of patches $i$ and $j$~\cite{ramachandran2019stand}:
\begin{align}
    \boldsymbol{A}^h_{ij}:=\operatorname{softmax}\left(\boldsymbol Q^h_i \boldsymbol K^{h\top}_j+\boldsymbol{v}_{pos}^{h\top} \boldsymbol{r}_{ij}\right)
\label{eq:local-attention}
\end{align}
Each attention head uses a trainable embedding $\boldsymbol{v}_{pos}^h \in \mathbb R^{D_{pos}}$, and the relative positional embeddings $\boldsymbol{r}_{ij}\in \mathbb R^{D_{pos}}$ only depend on the distance between pixels $i$ and $j$,  denoted denoted by a two-dimensional vector $\boldsymbol \delta_{ij}$. 

\begin{figure}[tb]
    \centering
    \begin{subfigure}[b]{.35\columnwidth}
    \includegraphics[width=\linewidth]{figs/photo_701.pdf}
    \caption{Input image}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=\linewidth]{figs/attention_map_init_nonlocal.pdf}
    \caption{Standard initialization}
    \end{subfigure}
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=\linewidth]{figs/attention_map_init_local_strength_0.5.pdf}
    \caption{Convolutional initialization, strength $\alpha=0.5$}
    \end{subfigure}   
    \begin{subfigure}[b]{\columnwidth}
    \includegraphics[width=\linewidth]{figs/attention_map_init_local_strength_2.pdf}
    \caption{Convolutional initialization, strength $\alpha=2$}
    \end{subfigure}
    \caption{\textbf{Positional self-attention layers can be initialized as convolutional layers.} (a): Input image from ImageNet, where the query patch is highlighted by a red box. (b),(c),(d): attention maps of an untrained SA layer (b) and those of a PSA layer using the convolutional-like initialization scheme of Eq.~\ref{eq:local-init} with two different values of the locality strength parameter, $\alpha$ (c, d). Note that the shapes of the image can easily be distinguished in (b), but not in (c) or (d), when the attention is purely positional.}
    \label{fig:maps-init}
\end{figure}

\paragraph{Self-attention as a generalized convolution}

\citet{cordonnier2019relationship} show that a multi-head PSA layer with $N_h$ heads and learnable relative positional embeddings~(Eq. \ref{eq:local-attention}) of dimension $D_{pos}\geq 3$ can express any convolutional layer of filter size $\sqrt N_h \times \sqrt N_h$, by setting the following:
\begin{align}
    \begin{cases}
    &\boldsymbol{v}_{pos}^{h}:=-\alpha^{h}\left(1,-2 \Delta_{1}^{h},-2 \Delta_{2}^{h}, 0,\ldots 0\right)\\ &\boldsymbol{r}_{\boldsymbol{\delta}}:=\left(\|\boldsymbol{\delta}\|^{2}, \delta_{1}, \delta_{2},0,\ldots 0\right)\\
    &\boldsymbol{W}_{q r y}=\boldsymbol{W}_{k e y}:=\mathbf{0}, \quad \boldsymbol{W}_{val}:=\boldsymbol{I}\\
    \end{cases}
    \label{eq:local-init}
\end{align}

In the above, 
\begin{itemize}[noitemsep]
    \item The \emph{center of attention} $\boldsymbol \Delta^h\in\mathbb{R}^2$ is the position to which head $h$ pays most attention to, relative to the query patch. For example, in Fig.~\ref{fig:maps-init}(c), the four heads correspond, from left to right, to $\boldsymbol \Delta^1 = (-1,1), \boldsymbol \Delta^2 = (-1,-1), \boldsymbol \Delta^3 = (1,1), \boldsymbol \Delta^4 = (1,-1)$.
    \item The \emph{locality strength} $\alpha^h>0$ determines how focused the attention is around its center $\boldsymbol \Delta^h$ (it can also by understood as the ``temperature'' of the softmax in Eq.~\ref{eq:attention}). When $\alpha^h$ is large, the attention is focused only on the patch(es) located at $\boldsymbol \Delta^h$, as in Fig.~\ref{fig:maps-init}(d); when $\alpha^h$ is small, the attention is spread out into a larger area, as in Fig.~\ref{fig:maps-init}(c). 
\end{itemize} 

Thus, the PSA layer can achieve a strictly convolutional attention map by setting the centers of attention $\boldsymbol \Delta^h$ to each of the possible positional offsets of a $\sqrt{N_h}\times \sqrt{N_h}$ convolutional kernel, and sending the locality strengths $\alpha^h$ to some large value. 
%As such, $\underset{h \in\left[N_{h}\right]}{\operatorname{concat}}\left[\text {SA}_{h}(\boldsymbol{X}_q)\right]$ will simply amount to the patch of pixels around patch $\boldsymbol X_q$, and $\boldsymbol W_{out}$ will function as a convolutional filter.

\section{Approach}

\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{figs/architecture.pdf}
    \caption{\textbf{Architecture of the ConViT.} The ConViT (left) is a version of the ViT in which some of the self-attention (SA) layers are replaced with gated positional self-attention layers (GPSA; right). Because GPSA layers involve positional information, the class token is concatenated with hidden representation after the last GPSA layer. In this paper, we typically take 10 GPSA layers followed by 2 vanilla SA layers. FFN: feedforward network (2 linear layers separated by a GeLU activation); $W_{qry}$: query weights; $W_{key}$: key weights; $v_{pos}$: attention center and span embeddings (learned); $r_{qk}$: relative position embeddings (fixed); $\lambda$: gating parameter (learned); $\sigma$: sigmoid function.}
    \label{fig:sketch}
\end{figure}

Building on the insight of~\cite{cordonnier2019relationship}, we introduce the ConVit, a variant of the ViT~\cite{dosovitskiy2020image} obtained by replacing a variable number of SA layers by a new type of layer which we call \emph{gated positional self-attention} (GPSA) layers. The core idea is to enforce the ``informed" convolutional configuration of Eqs.~\ref{eq:local-init} in the GPSA layers at initialization, then let them decide whether to stay convolutional or not. However, the standard parameterization of PSA layers (Eq.~\ref{eq:local-attention}) suffers from two limitations, which lead us two introduce two modifications.

\paragraph{Adaptive attention span} The first caveat in PSA is the vast number of trainable parameters involved, since the number of relative positional embeddings $\boldsymbol r_\delta$ is quadratic in the number of patches. This led some authors to restrict the attention to a subset of patches around the query patch~\cite{ramachandran2019stand}, at the cost of losing long-range information. 

To avoid this, we leave the relative positional embeddings $\boldsymbol r_\delta$ fixed, and train only the embeddings $\boldsymbol v^h_{pos}$ which determine the center and span of the attention heads; this approach relates to the \emph{adaptive attention span} introduced in~\citet{sukhbaatar2019adaptive} for Language Transformers. The initial values of $\boldsymbol r_\delta$ and $\boldsymbol v_{pos}^h$ are given by Eq.~\ref{eq:local-init}, where we take $D_{pos}=3$ to get rid of the useless zero components. Thanks to $D_{pos}\ll D_h$, the positional attention increases the parameter count by a marginal amount compared to the content attention.

\paragraph{Positional gating} 
The second issue with standard PSA the fact that the content and positional terms in Eq.~\ref{eq:local-attention} are potentially of different magnitudes, which can be problematic as the softmax will ignore the smallest of the two. In particular, the convolutional initialization scheme discussed above involves highly concentrated attention scores, i.e. high-magnitude values in the softmax. In practice, we observed that using a convolutional initialization scheme on vanilla PSA layers gives a boost in early epochs, but degrades late-time performance as the attention mechanism lazily ignores the content information (see SM.~\ref{app:without-gpsa}). 

To avoid this, GPSA layers sum the content and positional terms \emph{after} the softmax, with their relative importances governed by a learnable \emph{gating} parameter $\lambda_h$ (one for each attention head). Finally, we normalize the resulting sum of matrices (whose terms are positive) to ensure that the resulting attention scores define a probability distribution. The resulting GPSA layer is therefore parametrized as follows (see also Fig.~\ref{fig:sketch}):
\begin{align}
    \text{GPSA}_h(\boldsymbol{X}) :=& \operatorname{normalize}\left[\boldsymbol{A}^h\right] \boldsymbol{X} \boldsymbol{W}_{val}^h\\
    \boldsymbol{A}^h_{ij}:=&\left(1-\sigma(\lambda_h)\right) \operatorname{softmax}\left(\boldsymbol Q^h_i \boldsymbol K^{h\top}_j\right) \notag\\
    &+ \sigma(\lambda_h) \operatorname{softmax}\left(\boldsymbol{v}_{pos}^{h\top} \boldsymbol{r}_{ij}\right),
    \label{eq:gating-param}
\end{align}
where $\sigma:x\mapsto \nicefrac{1}{\left(1+e^{-x}\right)}$ is the sigmoid function, and $\left(\operatorname{normalize}\left[\bs A\right]\right)_{ij} = \bs A_{ij} / \sum_k \bs A_{ik}$. By setting the gating parameter $\lambda_h$ to a large positive value at initialization, one has $\sigma(\lambda_h)\simeq 1$ : the GPSA bases its attention purely on position, dispensing with the need of setting $\boldsymbol W_{qry}$ and $\boldsymbol W_{key}$ to zero as in Eq.~\ref{eq:local-init}. However, to avoid the ConViT staying stuck at $\lambda_h\gg 1$, we initialize $\lambda_h = 1$ for all layers and all heads.

\begin{table*}[h]
    \small
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \toprule
    Name & $N_h$ & $D_{emb}/N_h$ & Params (M) & Throughput & Top-1 & Top-5 & Top-1 (dist) & Top-5 (dist)\\
    \midrule
    DeiT-Ti\cite{touvron2020training}  & 3 & 64 & 5.7 & 2536 & 72.2 & - & 74.3 & - \\
    ConViT-Ti & 4 & 48 & 5.7 & 1102 & \textbf{73.1} & 91.7 & - & - \\
    \hline
    DeiT-S \cite{touvron2020training} & 6 & 64 & 22 & 940  & 79.8 & - & 80.9 & - \\
    ConViT-S & 9 & 48 & 27 & 382 & \textbf{81.3} & 95.7 & 82.9 & - \\
    \hline
    DeiT-B \cite{touvron2020training} & 16 & 64 & 86 & 292 & 81.8 & - & 83.0 & - \\
    ConViT-B & 16 & 48 & 86 & 161  & \textbf{82.4} & 95.9 & - & -\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Statistics of the models considered}. Throughput is the number of images processed per second on a V100 GPU, and top-1 accuracy is measured on ImageNet-1k test set without distillation (see SM.~\ref{app:distillation} for distillation). Notice that our ConViT-S outperforms the DeiT-B of~\cite{touvron2020training} with less parameters and higher throughput. Since we require the number of heads to be a perfect square to mimick a convolutional filter, we use a larger number of heads and embedding dimension (to maintain $D_{emb} = 64N_h$) than in~\citet{touvron2020training}. Therefore, we also compare our ConViTs to DeiTs of same architecture trained with the same hyperparameters, referred to as the ``Baseline'' models.
    }
    \label{tab:sizes}
\end{table*}


% \begin{table*}[h]
%     \small
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
%     \toprule
%     Name & $N_h$ & $D_{emb}$ & GPSA & Params (M) & Throughput & Top-1 & Top-5 & Top-1 (dist) & Top-5 (dist)\\
%     \midrule
%     DeiT-Ti\cite{touvron2020training}  & 3 & 192 & \xmark & 6 & 2536 & 72.2 & - & 74.3 & - \\
%     Baseline-Ti   & 4 & 256 & \xmark & 10   & 1769 & 75.9 & 93.2 & - & - \\
%     ConViT-Ti & 4 & 256 & \cmark & 10   & 1102 & \textbf{76.7} & 93.6 & - & - \\
%     \hline
%     DeiT-S \cite{touvron2020training}  & 6 & 384 & \xmark & 22 & 940  & 79.8 & - & 80.9 & - \\
%     Baseline-S   & 9 & 576 & \xmark & 48 & 480 & 79.0 & 94.4 & 82.5 & - \\
%     ConViT-S & 9 & 576 & \cmark & 48 & 382 & \textbf{82.2} & 95.9 & 82.9 & - \\
%     \hline
%     DeiT-B \cite{touvron2020training} & 12 & 768 & \xmark & 86 & 292 & 81.8 & - & 83.0 & - \\
%     Baseline-B  & 16 & 1024 & \xmark & 152 & 186  & 77.5 & 93.5 & - & -\\
%     ConViT-B & 16 & 1024 & \cmark & 152 & 161  & \textbf{82.5} & 95.9 & - & -\\
%     \bottomrule
%     \end{tabular}
%     \caption{\textbf{Statistics of the models considered}. Throughput is the number of images processed per second on a V100 GPU, and top-1 accuracy is measured on ImageNet-1k test set without distillation (see SM.~\ref{app:distillation} for distillation). Notice that our ConViT-S outperforms the DeiT-B of~\cite{touvron2020training} with less parameters and higher throughput. Since we require the number of heads to be a perfect square to mimick a convolutional filter, we use a larger number of heads and embedding dimension (to maintain $D_{emb} = 64N_h$) than in~\citet{touvron2020training}. Therefore, we also compare our ConViTs to DeiTs of same architecture trained with the same hyperparameters, referred to as the ``Baseline'' models.
%     }
%     \label{tab:sizes}
% \end{table*}

\paragraph{Architectural details}

Similar to language Transformers like BERT~\cite{devlin2018bert}, the ViT uses an extra ``class token", appended to the sequence of patches to predict the class of the input. Since this class token does not carry any positional information, the SA layers of the ViT do not use positional attention: the positional information is injected into the input before being propagated through the layers. Since GPSA layers involve positional attention, they are not well suited for the class token approach. We solve this problem by concatenating the class token to the representations after the last GPSA layer (see Fig.~\ref{fig:sketch})\footnote{We also experimented incorporating the class token as an extra patch of the image to which all heads pay attention to at initialization, but results were worse than concatenating the class token after the GPSA layers (not shown).}.

We based our ConVit on the DeiT~\cite{touvron2020training}, a data-efficient version of the ViT which has been open-sourced\footnote{ \url{https://github.com/facebookresearch/deit}}. Thanks to its ability to achieve competitive results without using any external data, it is both an excellent baseline and relatively fast to train: the largest model (DeiT-B) only requires two days of training on 8 GPUs with 32Gb RAM. Just like the ViT, the DeiT consists of 12 SA layers. Before being fed in, the images are sliced into non-overlapping patches of $16\times 16$ pixels, then embedded into vectors of dimension $D_{emb} = 64 N_h$ by a convolutional stem.

To mimic $2\times 2$, $3\times 3$ and $4\times 4$ convolutional filters, we consider three different models, with 4, 9 and 16 attention heads, denoted ConViT-Ti, ConViT-S and ConViT-B (see Tab.~\ref{tab:sizes}). The baseline against which they will be compared is the original DeiT of the same architecture but with vanilla SA layers instead of GPSA layers. Their number of heads differs from the DeiT-Ti ConViT-S and ConViT-B of~\citet{touvron2020training}, which respectively use 3, 6 and 12 attention heads: to avoid confusion, we will denote them as Baseline-Ti, Baseline-S and Baseline-B. 

\paragraph{Training details}

Since $D_{emb} = 64 N_h$, our models have a larger embedding dimension than the original DeiTs, and we lower the learning rate from $0.0005$ to $0.0004$ in order to maintain stable training for all models. To be able to train all our models on a single compute node, we set our batch size to 512.  We leave all other hyperparameters (data-augmentation, regularization, scheduling) presented in~\cite{touvron2020training} unchanged in order to achieve a fair comparison. Optimizing them for the ConViT may yield further improvements, the exploration of which we leave for future work.

Notice in Tab.~\ref{tab:sizes} that each ConViT has almost the same number of parameters as its Baseline, but lower throughput due to the positional attention. The difference is sizeable for small models (60\% slow-down for Tiny), but becomes smaller for larger models (15\% slow-down for Base). In spite of this slow-down, our ConViT-S (82.2\% top-1) outperforms the DeiT-B (81.8\% top-1) with less parameters and higher throughput. The same applies in presence of knowledge distillation where the ConViT-S reaches 82.9\% top-1, see SM~\ref{app:distillation}.

\section{Investigating the role of locality}
\label{sec:experimental}

In this section, we demonstrate that locality is naturally encouraged in standard SA layers, and examine how the ConViT benefits from locality being imposed at initialization.

\paragraph{SA layers are pulled towards locality}

We begin by investigating whether the hypothesis that PSA layers are naturally encouraged to become ``local" over the course of training~\cite{cordonnier2019relationship} holds for the vanilla SA layers used in ViTs, which do not benefit from positional attention. To quantify this, we define a measure of ``non-locality" by summing, for each query patch $i$, the distances $\Vert \boldsymbol \delta_{ij}\Vert $ to all the key patches $j$ weighted by their attention score $\boldsymbol A_{ij}$. We average the number obtained over the query patch to obtain the non-locality metric of head $h$, which can then be averaged to obtain the non-locality of the whole layer $\ell$:
\begin{align}
    D_{loc}^{\ell,h} &:= \frac{1}{L} \sum_{ij} \boldsymbol A^{h,\ell}_{ij} \Vert \boldsymbol \delta_{ij}\Vert, \notag\\
    D_{loc}^{\ell} &:= \frac{1}{N_h} \sum_h D_{loc}^{\ell,h}
    \label{eq:non-locality}
\end{align}
Intuitively, $D_{loc}$ is the number of patches between the center of attention and the query patch: the further the attention heads look from the query patch, the higher the non-locality. 

In Fig.~\ref{fig:distance}, we show how the non-locality metric evolves during training across the 12 layers of a DeiT-S trained for 300 epochs on ImageNet. During the first few epochs, the non-locality falls from its initial value in all layers, confirming that the DeiT becomes more ``convolutional". During the later stages of training, the non-locality metric stays low for lower layers, and gradually climbs back up for upper layers, revealing that the latter capture long range dependencies, as observed for language Transformers~\cite{sukhbaatar2019adaptive}. 

These observations are particularly clear when examining the attention maps (Fig.~\ref{fig:attn-nonlocal} of the SM), and point to the beneficial effect of locality in lower layers. In SM.~\ref{app:distillation}, we also show that the non-locality metric is lower when training with distillation from a convolutional network as in~\citet{touvron2020training},  suggesting that the locality of the teacher is partly transferred to the student~\cite{abnar2020transferring}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/nonlocality_nonlocal_small_IMNET.pdf}
    \caption{\textbf{SA layers are pulled towards locality.} We plot the non-locality metric defined in Eq.~\ref{eq:non-locality} (the higher, the further the heads look from the query pixel) throughout the training of a DeiT-S on ImageNet. Similar results for Baseline-Ti and DeiT-B are shown in SM.~\ref{app:non-locality}.}
    \label{fig:distance}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/gating_parameter_small_IMNET.pdf}
    \caption{\textbf{GPSA layers escape locality thanks to their gating parameters.} \textit{Left}: non-locality metric, see Eq.~\ref{eq:non-locality}. \textit{Right}: how much attention is paid to the content versus the positional information, calculated as $\E_h(1-\sigma(\lambda_h))$, see Eq.~\ref{eq:gating-param}. We trained a ConViT-S with 10 GPSA layers and 2 SA layers for 300 epochs on ImageNet. Similar results for ConViT-Ti and ConViT-B are shown in SM~\ref{app:non-locality}.}
    \label{fig:distance-nonlocal}
\end{figure}

\paragraph{GPSA layers escape locality}

In the ConViT, strong locality is imposed at the beginning of training through the convolutional initialization of the GPSA layers. In Fig.~\ref{fig:distance-nonlocal} (left), we see that this local configuration is escaped throughout training, as non-locality grows in each of the 10 GPSA layers. However, the lower layers retain some of the initial locality, as their final non-locality metric is lower than that of the SA layers (Fig.~\ref{fig:distance}).

In Fig.~\ref{fig:distance-nonlocal} (right), we show that the gating parameter gives more are more importance to content information throughout training, as $\E_h(1-\sigma(\lambda_h))$ increases in all layers. Its final value is around 0.5 in lower layers, which pay equal attention to content and position, whereas it is close to 1 in upper layers, where positional information is completely ignored.

\begin{figure*}[h!]
    \centering
    \begin{subfigure}[b]{.25\linewidth}
    \includegraphics[width=\linewidth]{figs/photo_701.pdf}
    \caption{Input image}
    \end{subfigure}   
    \begin{subfigure}[b]{.37\linewidth}
    \includegraphics[width=\linewidth]{figs/attention_map_final_701_nonlocal_tiny_IMNET.pdf}
    \caption{DeiT}
    \end{subfigure}
    \begin{subfigure}[b]{.37\linewidth}
    \includegraphics[width=\linewidth]{figs/attention_map_final_701_local_tiny_IMNET.pdf}
    \caption{ConViT}
    \end{subfigure}
    \caption{\textbf{The ConViT learns more diverse attention maps}. \textit{Left:} input image which is embedded then fed into the models. The query patch is highlighted by a red box and the colormap is logarithmic to better reveal details. \textit{Center:} attention maps obtained by a Baseline-Ti after 300 epochs of training on ImageNet. \textit{Right:} Same for ConViT-Ti. In each map, we indicated the value of the gating parameter in a color varying from white (for heads paying attention to content) to red (for heads paying attention to position). Attention maps for more images and more heads are shown in SM.~\ref{app:attention-maps}.}
    \label{fig:maps-final}
\end{figure*}

To understand the role of the various attention heads, we plot the attention maps of the DeiT and the ConViT at the end of training in Fig.~\ref{fig:maps-final}. For the ConViT, we also indicate the gating parameter of each attention head. In the upper layers (bottom row), the attention maps of DeiT and ConViT look qualitatively similar. In lower layers (top row), the attention maps of the ConViT are more varied: some heads pay more attention to content (heads 1 and 4) whereas other focus mainly on position (heads 2 and 3). Among the latter kind, some stay highly localized (head 3) whereas others broaden the attention span (head 2).

\begin{figure}[t]
    \centering
    \includegraphics[width=.36\columnwidth]{figs/strength.pdf}
    \includegraphics[width=.62\columnwidth]{figs/acc_vs_locality.pdf}
    % \includegraphics[width=.44\columnwidth]{figs/acc_vs_locality_dynamics.pdf}
    \caption{\textbf{The beneficial effect of locality}. \textit{Left:} Increasing the locality strength (i.e. how focused each attention head is its associated patch) and the number of GPSA layers, the final test accuracy achieved on the first 100 classes of ImageNet increases significantly. \textit{Right:} The beneficial effect of locality is particularly strong in the early epochs. 
    }
    \label{fig:strength}
\end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figs/ablation.pdf}
%     \caption{\textbf{Gating and convolutional initialization play nicely together.} We ran an ablation study on the first 100 classes of ImageNet. The baseline is the DeiT-S (pink). We experimented (i) replacing the 10 first SA layers by GPSA layers (``GPSA'') (ii) freezing the gating parameter of the GPSA layers (``frozen gate''); (iii) removing the local initialization (``conv''); (iv) freezing all attention module (``frozen''). The final top-1 accuracy of the various models trained is noted in the legend.}
%     \label{fig:ablation}
% \end{figure}

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
        Ref. & \thead{ Train \\ gating} & \thead{Conv \\init} & \thead{GPSA} & \thead{Train \\attention} & Top-1 \\
        \midrule
        ConViT & \cmark & \cmark & \cmark & \cmark & \textbf{82.2}\\
        (a) & \xmark & \cmark & \cmark & \cmark & 82.0\\
        (b) & \cmark & \xmark & \cmark & \cmark & 81.4\\
        (c) & \xmark & \xmark & \cmark & \cmark & 81.6\\
        Deit &       &        & \xmark & \cmark & 79.1\\
        (i) &       & \cmark & \cmark & \xmark & 78.6\\
        (ii) &       &        & \xmark & \xmark & 73.7\\
    \bottomrule
    \end{tabular}
    \caption{\textbf{Gating and convolutional initialization play nicely together.} We ran an ablation study on the ConViT-S trained for 300 epochs on the first 100 classes of ImageNet-1k. From the left column to right column, we experimented freezing the gating parameters to 0, removing the convolutional initialization, removing the GPSA layers altogether and freezing all attention modules.}
    \label{tab:ablation}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c}
%     \toprule
%         Model & Attention modules & Top-1 \\ \midrule
%         ConViT & Trained & 82.2 \\
%         ConViT & Frozen  & 78.6 \\
%         DeiT & Trained   & 79.1 \\
%         DeiT & Frozen    & 73.7 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:frozen_attn}
% \end{table}


\paragraph{Strong locality is desirable}

We next investigate how the performance of the ConViT is affected by two important hyperparameters of the ConViT: the \emph{locality strength}, $\alpha$, which determines how focused the heads are around their center of attention, and the number of SA layers replaced by GPSA layers. We examined the effects of these hyperparameters on ConViT-S, trained on the first 100 classes of ImageNet. As shown in Fig.~\ref{fig:strength}(a), final test accuracy increases both with the locality strength and with the number of GPSA layers; in other words, the more local, the better.

In Fig.~\ref{fig:strength}(b), we show how performance at various stages of training is impacted by the presence of GPSA layers. We see that the boost due to GPSA is particularly strong during the early stages of training: after 20 epochs, including 9 GPSA layers leads the test-accuracy to almost double, suggesting that the convolution initialization gives the model a substantial ``head start". This speedup is of practical interest in itself, on top of the boost in final performance.

\begin{figure*}[h]
    \centering
    % \begin{subfigure}[b]{\columnwidth}
    % \includegraphics[width=\linewidth]{figs/model_size_CIFAR10.pdf}
    % \caption{CIFAR10}
    % \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
    \includegraphics[width=\linewidth]{figs/model_size_CIFAR100_top1.pdf}
    \caption{CIFAR100}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
    \includegraphics[width=\linewidth]{figs/model_size_IMNET_top1.pdf}
    \caption{ImageNet-1k}
    \end{subfigure}
    \begin{subfigure}[b]{.31\textwidth}
    \includegraphics[width=\linewidth]{figs/data_size_top1.pdf}
    \caption{Subsampled ImageNet}
    \end{subfigure}
    \caption{\textbf{The convolutional inductive bias is particularly useful for large models applied to small datasets.} Each of the three panels displays the top-1 accuracy of the ConViTs and their corresponding DeiTs throughout training, as well as the relative improvement between the best top-1 accuracy reached by the DeiT and that reached by the ConViT. \textit{Left:} tiny, small and base models trained for 3000 epochs on CIFAR100. \textit{Middle:} tiny, small and base models trained for 300 epochs on ImageNet-1k. The relative improvement of the ConViT over the DeiT increases with model size. \textit{Right:} small model trained on a subsampled version of ImageNet-1k, where we only keep a fraction $f\in\{0.1,0.3,1\}$ of the images of each class. The relative improvement of the ConViT over the DeiT increases with the size of the dataset. 
    %For top-5 accuracies, see SM.~\ref{app:top5}.
    }
    \label{fig:performance}
\end{figure*}

\paragraph{Ablation study}
In Tab.~\ref{tab:ablation}, we present an ablation study where we experiment removing various ingredients from the ConViT: (a) the positional gating\footnote{To remove gating, we freeze all gating parameters to $\lambda=0$ so that the same amount of attention is paid to content and position.}, (b) the convolutional initialization, (c) both (a) and (b) and finally the GPSA altogether (which leaves us with a DeiT).

Surprisingly, GPSA alone (c) already brings a substantial benefit over the DeiT (+2.5 top-1), demonstrating the importance of positional attention. Adding the convolutional initialization (a) yields further improvement (+2.9), which becomes even stronger when training the gating parameters (ConViT, +3.1). Interestingly, gating is useful in presence of the convolutional initialization, but lowers performance otherwise as (b) performs worse than (c).

We also investigated the performance of models with all attention modules frozen, leaving only the patch embeddings and FFNs to be trained. As expected, performance of the DeiT (ii) is strongly degraded (-5.4). However, the ConViT (i) is less affected (-3.6) and reaches a performance remarkably close to the vanilla DeiT thanks to the convolutional initialization.

\section{Performance of the ConViT}

In this section we demonstrate the improvement resulting from the soft convolutional inductive biases. In all experiments, we use a ConViT with 10 GPSA layers followed by 2 SA layers, and use a locality strength $\alpha=1$, following the results presented in the previous section.

\paragraph{Dependence on model size}

We first investigate how the benefit of GPSA scales with model size. In Fig.~\ref{fig:performance}(a,b), we display the results of the three models described in Tab.~\ref{tab:sizes} trained for 300 epochs on CIFAR100 and ImageNet\footnote{For CIFAR100, we rescaled the images to $224\times 224$ and increased the number of epochs (adapting the learning rate schedule correspondingly) to mimic the ImageNet scenario.}. For both datasets, the ConVits outperforms their baselines (DeiTs of same architecture). The relative improvement increases as the model grows larger, ranging from 4\% (tiny) to 12\% (base) on CIFAR100. On ImageNet, the improvements are smaller but still range from 1\% (tiny) to 6\% (base). 

Note that our ConViT is compatible with the distillation methods introduced in~\citet{touvron2020training} at no extra cost. As shown in~\ref{app:distillation}, hard distillation improves performance, enabling the ConViT-S to reach 82.9\% top-1 accuracy, on the same footing as the hard-distilled DeiT-B with half the number of parameters.

\paragraph{Dependence on sample size}

To investigate the sample-efficiency of the ConViT in a systematic way, we subsample each class of the ImageNet-1k dataset by a fraction $f=\{0.1,0.3,1\}$ and observe how performance is impacted in Fig.~\ref{fig:performance}(c), adapting the number of epochs and learning rate schedule such that the total number images presented to the model is the same in all cases. 

As one might expect, the top-1 accuracy of both the DeiT and its ConVit counterpart drops as $f$ decreases. However, the ConViT suffers much less: When keeping only 10\% of the training data, the ConVit achieves 58.6\% top-1 accuracy, versus 45.9\% for its DeiT counterpart (see Tab~\ref{tab:perfs}). This result can be directly compared to~\cite{zhai2019s4l}, which after testing several thousand convolutional models reach a top-1 accuracy of 56.4\% ; the ConViT is therefore highly competitive in terms of sample efficiency.

Together with Fig.~\ref{fig:performance}(a,b), these findings confirm our hypothesis that the convolutional inductive bias is most helpful for large models applied to small datasets, i.e. in the highly underspecified regime, as depicted in Fig.~\ref{fig:phase_space}.


\section{Conclusion and perspectives}

The present work investigates the importance of initialization and inductive biases in learning with Transformers. By showing that one can take advantage of convolutional constraints in a soft way, we merge the benefits of architectural priors and expressive power. The result is a simple recipe that improves trainability and sample efficiency, without increasing model size or requiring any tuning. 

Our approach can be summarized as follows: instead of interleaving convolutional layers with SA layers as in hybrid models, let the layers decide whether to be convolutional or not by adjusting the gating parameter. More generally, combining the biases of varied architectures and letting the model choose which ones are best for a given task is a promising direction, which reduces the need for greedy architectural search while increasing interpretability. In future work, we aim to investigate this theme further by studying various mixtures of initialization schemes incorporating other aspects of convolutional networks. 

%One of our long-term goals is to utilize our understanding of how a neural network learns to classify data to design more interpretable and explainable AI systems.
%From a theoretical point-of-view, one of the challenges in deep learning is understanding how a given dataset with a particular structure matches the architecture's internal biases.  


%In future work, we aim to investigate this theme further by studying ``informed initialization" deeper: instead of initializing the ViT as an untrained CNN, could one initialize it as a partially trained CNN, then fine-tune on it?

%could one, for example, initialize the fully-connected layers between the self-attention layers such that they behave like pooling layers?


